Pattern analysis in a benthic bacteria-nutrient system

We study pattern formation in a reaction-diffusion system for a benthic bacteria-nutrient model in a marine sediment, which originally contains some spatially varying coefficients and with these shows some layering of patterns. Using the Landau reduction for the system with homogeneous coefficients, we locally analyze Turing bifurcations in 1D and 2D. Moreover, we use the software pde2path to compute the corresponding branches globally and find a number of snaking branches of patterns over patterns. This shows that spatially varying patterns are not necessarily due to spatially varying coefficients. We find a type of hexagon patches on a homogeneous background with no prior mention in the literature. We show the first numerically calculated solution-branch, which connects two different types of hexagons in parameter space. We call states on this branch rectangles. We check numerically, if the stability changes for hexagons and stripes, which are continued homogeneously into the third dimension. We find that stripes and one type of hexagons have the same stable range over bounded 2D and 3D domains, while the other type of hexagons becomes unstable earlier. Here we find a snaking branch of solutions, which are spatial connects between hexagonal prisms and a genuine 3D pattern (balls).

==> Reports/report1 <==
 2014-10-30 Thu 6:44:29:180 PM
-----------------------------------------------------------------------------------
Subject: Finalized Report
Synopsis: The author discusses a previously published semilinear diffusion-reaction system that arises in the modeling of interactions between benthic bacteria and nutrient. The pattern analysis, carried out using heavy analytical techniques and numerical tools, is quite involved and very detailed and it emerges a very rich behaviour in dependence of parameters.

Assessment: The author gives, what appears to be a quite extensive of the picture of the dynamics of the system. My main qualm with the paper is the following: the model studied here is taken from the literature matter of factly without explanation an discussion of model assumptions. I would assume that the sediment is a porous medium. Under which conditions is it justified to neglect the flow field? What is the interpretation of diffusion in this system Ã¢?? is it accounted for that part of the domain is filled by solid material? Since the model was published before, I don't expect a big and detailed description and justification of the model, but I would have hoped for some guidance to the reader to get a better understand the physical and biological scenario. Also, in (1) the growth and uptake rate functions are more complicated than what we often see. I would like to see this discussed in some more detail. How do these terms arise? How much of the richness in model behavior is due to the term u/(k+u)? Does the analysis (and results) simplify much in the more familiar case \gamma=1?
In a similar vein, but probably in more detail, I would have like to see a discussion whether the different patterns that are observed have a biological meaning/interpretation and whether they lead to new insight about the biological system. In (6) and throughout the text, for dimensional parameters, dependent and independent variable, I would like to see units. Otherwise, I think the work is conducted quite well. To pull this through requires quite some endurance.


